Decohering Tensor Network Quantum Machine Learning Models

Tensor network quantum machine learning (QML) models are promising applications on near-term quantum hardware. While decoherence of qubits is expected to decrease the performance of QML models, it is unclear to what extent the diminished performance can be compensated for by adding ancillas to the models and accordingly increasing the virtual bond dimension of the models. We investigate here the competition between decoherence and adding ancillas on the classification performance of two models, with an analysis of the decoherence effect from the perspective of regression. We present numerical evidence that the fully-decohered unitary tree tensor network (TTN) with two ancillas performs at least as well as the non-decohered unitary TTN, suggesting that it is beneficial to add at least two ancillas to the unitary TTN regardless of the amount of decoherence may be consequently introduced.

==> arXiv v2/preamble.tex <==
\usepackage[pdftex, breaklinks=true]{hyperref}
\hypersetup{
    pdffitwindow=true,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of the page to the window
    pdfnewwindow=true,      % links in new PDF window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=red,      % color of internal links (change box color with linkbordercolor)
    citecolor=blue,        % color of links to bibliography
    urlcolor=blue           % color of external links
}
\usepackage[utf8]{inputenc}
\DeclareSymbolFont{slenderlargesymbols}{OMX}{ccex}{m}{n}
\DeclareMathSymbol{\prod}{\mathop}{slenderlargesymbols}{"51}
\usepackage{amsfonts, amssymb, amsmath}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{braket} 
\usepackage{multirow}
\usepackage[T1]{fontenc}
\usepackage{bbm}
\usepackage{float}
\usepackage{caption}
\usepackage{subcaption}

\newcommand{\ketbra}[2]{|#1\rangle \langle#2|}

\def\tablename{Table}   % so that table caption is in small case

\newtheoremstyle{cited}%
  {3pt}% (space above)
  {3pt}% (space below)
  {\itshape}% (body font)
  {}% (indent amount)
  {\bfseries}% {theorem head font}
  {.}% {punctuation after theorem head}
  {.5em}% {space after theorem head}
  {\thmname{#1} \thmnumber{#2} \thmnote{\normalfont#3}}% {theorem head spec}
\theoremstyle{cited}
\newtheorem{citedprop}{Proposition}

% \renewcommand\bra[1]{{\langle{#1}|}}
\makeatletter
% \renewcommand\ket[1]{%
%   \@ifnextchar\bra{\k@t{#1}\!}{\k@t{#1}}%
% }

\newcommand\k@t[1]{{|{#1}\rangle}}
\makeatother
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclareMathOperator{\Tr}{\text{Tr}}
\DeclareMathOperator{\EX}{\mathbb{E}}% expected value

\usepackage{xcolor}
\newcommand{\correct}[1]{{\color{red} #1}}
\usepackage[normalem]{ulem}
\newcommand{\remove}[1]{{\color{red} \sout{#1}}}
\newcommand{\bw}[1]{{\color{red} #1}}
\newcommand{\haoran}[1]{{\color{blue} #1}}
\newcommand{\haorancomment}[1]{{\color{green} #1}}

\newcommand{\add}[1]{{\color{red} #1}}
\newcommand{\modified}[1]{{\color{blue} #1}}

\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{coro}{Corollary}
\newtheorem{lemma}{Lemma}

\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing}
\makeatletter
\def\underbrace#1{%
   \@ifnextchar_{\tikz@@underbrace{#1}}{\tikz@@underbrace{#1}_{}}}
\def\tikz@@underbrace#1_#2{%
   \tikz[baseline=(a.base)] {\node[inner sep=2] (a) {\(#1\)};
   \draw[line cap=round,decorate,decoration={brace,amplitude=4pt}]
     (a.south east) -- node[pos=0.5,below,inner sep=7pt] {\(\scriptstyle #2\)} (a.south west);}}
 
\def\overbrace#1{%
   \@ifnextchar^{\tikz@@overbrace{#1}}{\tikz@@overbrace{#1}^{}}}
\def\tikz@@overbrace#1^#2{%
   \tikz[baseline=(a.base)] {\node[inner sep=2] (a) {\(#1\)};
   \draw[line cap=round,decorate,decoration={brace,amplitude=4pt}]
     (a.north west) -- node[pos=0.5,above,inner sep=7pt] {\(\scriptstyle #2\)} (a.north east);}}
\makeatother

\setcounter{secnumdepth}{2} %Index sections for reference

\usepackage{siunitx}
% \usepackage{geometry}
% % \newgeometry{top=2.9cm,bottom=2.9cm,left=2.9cm,right=2.9cm}
% % \newgeometry{margin=1.25in}




% ********************* added for one column footnote <<<<<<<<<<<<<<<<<<<<
\makeatletter 
    
\renewcommand\onecolumngrid{% <<<<<<
\do@columngrid{one}{\@ne}%
\def\set@footnotewidth{\onecolumngrid}% <<<<<<<<<<<<<<<<
\def\footnoterule{\kern-6pt\hrule width 1.5in\kern6pt}%
}

\renewcommand\twocolumngrid{% <<<<<<
        \def\footnoterule{% restore rule
        \dimen@\skip\footins\divide\dimen@\thr@@
        \kern-\dimen@\hrule width.5in\kern\dimen@}
        \do@columngrid{mlt}{\tw@}
}%

\makeatother    
%%  *********************************************** 
